Facilitating Self-monitored Physical Rehabilitation with Virtual Reality and Haptic feedback

Physical rehabilitation is essential to recovery from joint replacement operations. As a representation, total knee arthroplasty (TKA) requires patients to conduct intensive physical exercises to regain the knee's range of motion and muscle strength. However, current joint replacement physical rehabilitation methods rely highly on therapists for supervision, and existing computer-assisted systems lack consideration for enabling self-monitoring, making at-home physical rehabilitation difficult. In this paper, we investigated design recommendations that would enable self-monitored rehabilitation through clinical observations and focus group interviews with doctors and therapists. With this knowledge, we further explored Virtual Reality(VR)-based visual presentation and supplemental haptic motion guidance features in our implementation VReHab, a self-monitored and multimodal physical rehabilitation system with VR and vibrotactile and pneumatic feedback in a TKA rehabilitation context. We found that the third point of view real-time reconstructed motion on a virtual avatar overlaid with the target pose effectively provides motion awareness and guidance while haptic feedback helps enhance users' motion accuracy and stability. Finally, we implemented \systemname to facilitate self-monitored post-operative exercises and validated its effectiveness through a clinical study with 10 patients.

==> sections/5_system_characterization.tex <==
\section{System Characterization}
\label{sec:characterization}

Based on the factors discussed in Section~\ref{sec:system_design}, we conducted two user studies to characterize \systemname's optimal visual and haptic feedback design respectively to facilitate physical rehabilitation exercises.
We then present our final system implementation based on the findings. 

% In achieving self-monitoring, virtual reality based headsets are used for displaying the target rehabilitation poses and the kinetic reconstruction enabled by the IMU sensor straps worn around the thigh and the ankle. 
% In this section we explore different varieties of visual displays in the virtual reality to provide clear, convenient, and comfortable visual display for rehabilitation sessions. 
% Specifically, we studied how first or third point of view affect visual information delivery and how the presence of virtual hands, in lieu of the patient, might impact patients' performance through establishing virtual authority.

\subsection{Characterizing the visual feedback}
\label{sec:visual}

% We conducted a user study to characterize the visual system by controlling two factors(point of view and hand clues) and comparing the performance of users.
We investigate the factors \textbf{point of view} and \textbf{presence of authority} (i.e., virtual hands) to further characterize the visual feedback.

\subsubsection{Design}

% Past studies affirm that first point of view brings immersion which is crucial to self-motivated rehabilitation []. 
Based on the design of the visual system in Section~\ref{sec:visual_design}, we evaluated four conditions with two factors in this study: \textbf{TPH}: third point of view with virtual hands, \textbf{TPN}: third point of view without virtual hands, \textbf{FPH}: first point of view with virtual hands, and \textbf{FPN}: first point of view without virtual hands.
Examples of all conditions for the pose \textit{bed-supported knee bends} are provided in Fig~\ref{fig:visual_conditions}. 
We set the target poses based on Section~\ref{observation}, which is 30 degrees for \textbf{straight leg raises} and \textbf{prone leg raises}, 90 degrees for \textbf{bed-supported knee bends}.
We counter-balanced the order of the conditions by a latin-square, and the order of the poses to be performed in each condition is randomized. 

\begin{figure}[htbp]
     \centering
     \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/tph.PNG}
        \caption{\textbf{TPH}: third point of view with hand clues}
        \label{fig:tph}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/tpn.PNG}
        \caption{\textbf{TPN}: third point of view without hand clues}
        \label{fig:tpn}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/fph.PNG}
        \caption{\textbf{FPH}: first point of view with hand clues}
        \label{fig:fph}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/fpn.PNG}
        \caption{\textbf{FPN}: first point of view without hand clues}
        \label{fig:fpn}
     \end{subfigure}
     \caption{Illustration of four different visual feedback conditions.}
     \label{fig:visual_conditions}
\end{figure}

\subsubsection{Participants}
We recruited 16 participants (6 females, 10 males) from a local university with an average age of 21.5 (SD = 2.3) and an average self-reported familiarity to VR of 2.88 (SD = 1.4) out of 5 ($1$: Not familiar at all; $5$: Very familiar). 
None had perception disorders or vision problems. We tested half of the participants' left legs and the rest's right legs. Each participant received a 15 USD compensation for the 40-minute study. 

\subsubsection{Apparatus}
% this is system hardware setup and implementation
% quest model info
We used the IMUs straps (see Section~\ref{sec:motiontracking}) for accurate motion tracking.
We developed a VR application with Unity using the Oculus Quest 2~\footnote{https://www.oculus.com/quest-2/} headset with a desktop computer (Intel 16-Core i7 CPU@3.30 GHz, 32 GB RAM, NVIDIA GeForce RTX 3080 GPU).
The IMUs' data was transmitted to the VR application via Bluetooth. 

% The virtual avatar is displayed in a default white background. 
% We projected the tracking data obtained from the two IMU sensors on the thigh and the calf onto the leg movement of an avatar in the virtual environment. 
% For each exercise, a semi-transparent leg representing the target position is overlaid onto the avatar to provide an intuitive visual representation of the motor learning goal for a specific motion. 
% A text that floats above the virtual avatar displays the current count of the movements and the total movements to be completed in an exercise. 
% When the system detects that the user reaches the target pose based on the tracking, a countdown of 10 seconds starts on the screen. 
% Figure (?) shows an example scene of the VR display that the user sees during a session. 

\subsubsection{Procedure}
We conducted the user study in a lab environment. 
Participants were first informed of the study purpose and the procedure. 
After providing the demographic information, they were instructed to sit on a yoga mat.
The researchers helped the participants wear the IMU straps and the VR headset.
% They were then shown a sample scene to familiarize themselves with the representation of the virtual avatar, the semi-transparent target leg with or without the guiding virtual hands depending on the condition. 
Participants familiarized themselves with the VR environment and the virtual avatar.
% We counterbalanced the conditions for each participant. 
We tested three postures with 5 repetitions in each test session. 
Therefore, each participant performed $4$ conditions/sessions $\times$ $3$ exercise postures $\times$ 5 repetitions $= 60$ movements in this user study.
% The participant started reaching his/her leg to the target pose once the session began.
% % When the participant understands the target, he or she takes the baseline and then starts moving.
% When the participant reached the maximum/target position and stabilized the pose, the 10-second countdown automatically started.
% When the countdown ended, the participant could move his/her leg back to the ready posture. The participant could rest for 5 seconds and start the next repetition. 
The experimenter helped the participant to get ready for the next exercise posture with postures' order counterbalanced. 

After each session, the participant was asked to grade the following five statements using a 5-point Likert scale (1: strongly disagree, 3:neutral, 5: strongly agree): \textit{"I could quickly understand the visual instructions"} (information presentation), \textit{"I was well aware of my motions"} (self-perception), \textit{"I felt motivated"} (motivation), \textit{"I felt stressed"} (stress), and \textit{"I had a good experience exercising with the system"} (overall impression).
Users took a 5-minute break between sessions. 
After all the sessions were completed, participants could revise and modify their scores for the 4 conditions. Lastly, we conducted a 5-minute interview to investigate their opinions on the visual feedback features. 

\subsubsection{Results}
% objective and subjective
As mentioned in Section~\ref{sec:segmentation}, we evaluated the following objective metrics.

\begin{enumerate}
    \item \textbf{Understanding time} is the duration of the understanding phase when they see a posture for the first time in a session. This indicates the time taken to understand the new instructions given. 
    % We consider the understanding phase of the posture's rest 4 repetitions for unindicative due to the learning effect.
    \item \textbf{Angle deviation} is the angular difference between the starting pose of the holding phase and the target pose. The starting pose is the participant's pose at the instant when the 10-second countdown starts. Without the effect of fatigue during the holding, this metric measures how accurately participants can achieve the target pose with the system.
    \item \textbf{Effective time} is the duration within the 10-second holding phase in which the participant stably holds the starting pose without large-scale fluctuations. We defined a threshold of 4-degree deviation ($\pm 2$ degrees) within which the holding is stable and effective. This metric is indicative of the stability of the holding phase. 
    % In quantifying the stability of the pose during the holding phase, we defined a threshold of 4-degree fluctuation (($\pm 2$) degrees away from the pose during the holding phase) fluctuation from the measurements when the countdown started is acceptable. Within this range we define the pose to be stable and effectively held. We thus measure stability by evaluating the effective time within 10 seconds that the participants stayed in their acceptable fluctuation range.
\end{enumerate}

The variables for the objective metrics did not follow a normal distribution ($p < 0.05$ under Shapiro–Wilk Test for all tested variables).
We thus used Wilcoxon signed-rank test ($p < 0.05$) for statistic analysis on the objective metrics and the subjective evaluation.
% Thus a non-parametric analysis of variance based on the Aligned Rank Transform was used to evalte objective and subjective data. 

\begin{figure}[htbp]
     \centering
     \begin{subfigure}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/visualacc.png}
        \caption{}
        \label{fig:visualacc}
     \end{subfigure}
     \hspace{3em}
     \begin{subfigure}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/visualeff.png}
        \caption{ }
        \label{fig:visualeff}
     \end{subfigure}
     \hspace{3em}
     \begin{subfigure}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/visualunder.png}
        \caption{ }
        \label{fig:visualunder}
     \end{subfigure}
     \caption{Objective results of the visual feedback characterization study.}
     \label{fig:visual}
\end{figure}

% \textit{Users take similar amount of time to understand the task with different point of views and hand clues.}
% The test results showed no significant difference between \textbf{TPH} $(M = 13.57, SD = 12.31)$, \textbf{TPN} $(M = 20.93, SD = 21.44)$, \textbf{FPH} $(M = 17.89, SD = 19.61)$ and \textbf{FPN} $(M = 14.27, SD = 18.68)$.

Statistical analysis results revealed a significant effect of the \textbf{point of view} on the \textit{understanding time} $(Z = 7.03, p < 0.001)$. 
This indicates that users take much less time to understand the instructions using the third point of view in VR. 
Fig~\ref{fig:visual} shows no significant effect of other factors on the objective metrics. 


% Understanding time
% significant effect  on understanding time of pov*hand interaction. A($M=13.56632, SD=12.31194$) B($M=20.93497, SD=21.44257$) C($M=17.89547, SD=19.60763$) D($M=14.27465, SD=18.68244$)

% \textit{The point of view and the virtual hand do not affect the accuracy of the pose.}
% The test results showed no significant difference between \textbf{TPH} $(M = 5.67, SD = 5.99)$, \textbf{TPN} $(M = 4.99, SD = 5.40)$, \textbf{FPH} $(M = 4.82, SD = 3.28)$ and \textbf{FPN} $(M = 4.64, SD = 3.91)$.

% Angle
% no significant effect on angle accuracy was found. A($M=5.670875, SD=5.989775$) B($M=4.988812, SD=5.399497$) C($M=4.818708, SD=3.27802$) D($M=4.642636, SD=3.905585$)

% \textit{Users could find their motion's deviation and correct it better with a third point of view. While the presence of hand clues have a negative effect.}
% On the metric of time proportion, point of view had significant impact $(F_{1, 937} = 8.21, p < 0.05)$.
% However, the hand clues had a negative significant influence on angle accuracy $(F_{1, 937} = 16.38, p < 0.05)$.
% After the experiment, several participants reported that the presence of hand clues obstructed their observation to the target pose.

% Proportion within the range
% significant effect of pov ($F=8.2138, p<0.01$) , hand ($F=16.3763, p<0.001$) and pov*hand interaction ($F=13.1920, p<0.001$). A($M=4.540571, SD=4.363222$) B($M=4.644591, SD=4.312741$) C($M=2.59811, SD=3.649957$) D($M=4.861772, SD=4.338522$)

% Need a figure

% Q6: significant difference ($F=10.52311, p<0.01$) between A($M=4.4375, SD=0.892094913$) B($M=4.5625, SD=0.62915287$) and C($M=4.0625, SD=0.771902412$) D($M=3.875, SD=0.718795288$)
%(self-perception) The assessment of the questions related to the user's self-perception indicates statistically significant effect of the point of view factor on the question "To what extent did you feel that you know how your leg moved in the virtual environment" (p < 0.01), and it is in favor of the third point of view. 

\begin{figure}[htbp]
     \centering
     \begin{subfigure}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/visualinf.png}
        \caption{ }
        \label{fig:visualinf}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/visualperp.png}
        \caption{ }
        \label{fig:visualperp}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/visualmot.png}
        \caption{ }
        \label{fig:visualmot}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/visualstr.png}
        \caption{ }
        \label{fig:visualstr}
     \end{subfigure}
     \begin{subfigure}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/visualove.png}
        \caption{ }
        \label{fig:visualove}
     \end{subfigure}
     \caption{Subjective results of the visual feedback characterization study.}
     \label{fig:visualsub}
\end{figure}

% Information presentation: tpov > fpov
% Self perception: tpov > fpov
% motivated: none
% stress: tpov > fpov
% overall: tpov > fpov

As shown in Fig~\ref{fig:visualsub}, statistical analysis results indicated that the third point of view significantly outperforms the first point of view on \textit{information presentation} ($Z = 2.69, p < 0.01$), \textit{self perception} ($Z = 4.12, p < 0.001$), \textit{stress} ($Z = 2.15, p = 0.032$), and \textit{overall impression} ($Z = 2.92, p < 0.01$). However, there is no statistical significant effect of \textbf{presence of authority} on the qualitative metrics. 

% The quality of information presentation and the clarity of self-perception, which indicates awareness of one's own motions, were both rated higher for third point of view. 
% Participants also reported a higher level of stress when exercising with third of point view, indicating that they felt more compelled to comply with the instructions. 
% Participants preferred third point of view over first point of view overall. No other factor or metric was significant.

% \textit{Third point of view make users perceive their motion better.}
% For the self-perception metric, users perceived their motion better with third point of view as \textit{TPH} $(M = 4.44, SD = 0.89)$ and \textit{TPN} $(M = 4.56, SD = 0.63)$ was significantly higher $(F_{1,60} = 10.52, p < 0.05)$ than \textit{FPH} $(M = 4.06, SD = 0.77)$ and \textit{FPN} $(M = 3.88, SD = 0.72)$.
% The hand clues did not significantly affect the results of self perception.

% \textit{Users are more motivated with the third point of view.}
% Third point of view could motivate users completing tasks better as \textit{TPH} $(M = 4.31, SD = 0.79)$ and \textit{TPN} $(M = 4.25, SD = 0.77)$ was significantly higher $(F_{1, 60}=4.12, p < 0.05)$ than \textit{FPH} $(M = 4.13, SD = 0.72)$ and \textit{FPN} $(M = 3.88, SD = 0.89)$.
% The hand clues did not significantly affect the metric of motivation.

%Q8: significant difference ($F_{1,60}=4.11693, p<0.05$) between A($M=4.3125, SD=0.793200269$) B($M=4.25, SD=0.774596669$) and C($M=4.125, SD=0.718795288$) D($M=3.875, SD=0.885061203$)
%(motivation)Similarly, the assessment of the questions related to the user's motivation indicates statistically significant effect of point of view on the question "To what extent were you satisfied with your performance" (p < 0.05), and it is also in favor of the third point of view. 
14 out of 16 participants indicated in the interviews that they found the third point of view more suitable for physical rehabilitation poses. They claimed that the third point of view offers a clearer and more complete view of their bodies without demanding extra physical effort, especially for the pose prone leg raises.
% This is especially significant during the pose prone leg raises in which participants had to turn around to see their own body under the first point of view.
% The insignificant effect of virtual hands on both the objective and subjective metrics were confirmed during the interview. 15 out of 16 participants reported that the presence of virtual hands made not much of a difference.
% Some participants also reported that the virtual hands and the avatar with the reconstructed motion are sometimes obstructing each other in both the first and the third point of view.

In summary, results revealed that \systemname should adopt the third point of view without the virtual hand.

% According to our results, third point of view offers more information of the user's current posture, which enhances their self-perception and motivation. 
% While the presence of authoritative hands had impact on a certain pose, the subjective data suggest that the majority of the subjects believed it didn't help them in any way. 
% Therefore, the final visual system is in third point of view, with no appearance of virtual hands.


\subsection{Characterizing the haptic feedback}
\label{sec:haptic}
We investigate different haptic methods to further characterize the visual feedback.

\subsubsection{Design}
We evaluated three conditions: \textbf{None}: no haptic feedback, \textbf{Vibro}: vibrotactile feedback, and \textbf{Pneu}: pneumatic feedback. 
All visual display setup is kept the same as the VR-based visual feedback characterized in Section~\ref{sec:visual}.
% We additionally asked the participants to evaluate the effectiveness of the haptic guidance in the two haptic conditions and
Other study designs were kept the same as the previous study. 
% We counter-balanced the order of the conditions by a latin-square and the order of the poses to be performed in each condition is randomized. 

% A: None
% B: Vibro
% C: Pneu

\subsubsection{Participants}
We recruited 11 participants (5 females, 6 males) from a local university with an average age of 24.1 ($SD = 4.0$) and an average self-reported familiarity to VR of 2.18 ($SD = 1.0$) out of 5 ($1$: Not familiar at all; $5$: Very familiar).
None had perception disorders or vision problems.
We tested 6 of the participants' left legs and the rest's right legs.
Each participant received a 15 USD compensation for the 40-minute study.

\subsubsection{Apparatus}
The hardware setup of the visual system remains the same as the study in section~\ref{sec:visual}. 
We prototyped two feedback straps to be worn at the thigh and the calf for both the vibrotactile and the pneumatic feedback.
Each feedback strap had vibrotactile actuators or pneumatic air compartments at the up and down sides of the strap to provide up and down directional feedback.
Both systems receive commands for actuating the haptic feedback from the computer via serial ports.
The vibrotactile actuators(9000 rpm) were screwed directly onto the elastic straps.
A total of four vibrators for a set of the vibrotactile haptic systems was powered and controlled by an Arduino Uno connected to the computer. 
We adopted the proposed fabrication method for prototyping inflatable structures in aeroMorph~\cite{ou_16}.
% Thick Thermoplastic polyurethane(TPU) coated nylon fabric was used to create air compartments in conjunction with a heat sealer to manually seal the air compartments. 
Fabricated air compartments of 7cm wide and 8cm long were glued to the inner side of the straps, so the air compartments are in contact with the skin.
% 1 meter of silicone tube (ID, OD) is attached to each air compartment through silicone tube fittings and o-rings.
% 4 tubes for one set of thigh and leg straps are routed together through the strap. 
% Through a Y-shaped three way connector, the other end of the tube is connected to another two silicone tubings (ID, OD) which connects to two micro pumps (12 V, 5 W), 
Each air compartment was controlled by two micro-pumps (12 V, 5 W), one for inflation and one for deflation. 
A  total of 8 micro-pumps were controlled by an 8-way relay and an Arduino Mega~\footnote{https://www.arduino.cc/en/Main/arduinoBoardMega2560} connected to the computer. 
The micro-pumps were powered by a regulated power supply and a step-down converter. 
When fully inflated, each air compartment exerted a force of around 10N on the skin. 

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.4\linewidth]{figures/characterization/pneumatic.jpg}
%     \caption{The inflated air compartment.}
%     \label{fig:pneu}
% \end{figure}

\subsubsection{Procedure}
The study procedure was similar to the one in section~\ref{sec:visual}. 
With the help of researchers, the participants wore IMU straps, vibrotactile/pneumatic feedback straps, and the VR headset for this study.
We tested three postures (straight leg raises, prone straight leg raises, and bed-supported knee bends as illustrated in Fig.~\ref{fig:poses}) with 5 repetitions in each test session. Therefore, each participant performed $3$ conditions/sessions $\times$ $3$ exercise postures $\times$ 5 repetitions $= 45$ movements in this user study. 

\subsubsection{Results}
% Meanwhile, the participants’ correctness of the motion, the time to understand the information, and time taken to complete the motion.
% We used the same statistical analysis method in the visual characterization experiment since the quantitative and qualitative metrics are the same type.
We adopted the same objective and subjective metrics and the statistical analysis methods as Section~\ref{sec:visual}.
%The objective and subjective metrics evaluated remain the same as Section~\ref{sec:visual_design}.
%We used non-parametric Friedman test ($p < 0.05$) along with the Conover post-hoc test ($p < 0.05$) for statistic analysis on the objective metrics and Friedman test with Wilcoxon signed-rank post-hoc test ($p < 0.05$) for the subjective evaluation.

% After validating that the variables did not follow a normal distribution ($p < 0.05$ under Shapiro–Wilk Test for all tested variables), the Friedman test along with the Conover post-hoc test was applied, since the analysis involving the comparison of all three conditions. 
% We analyzed the answers to the survey and the objective data collected by the system. 
% As the variables did not follow a normal distribution ($p < 0.05$ under Shapiro–Wilk Test for all tested variables), a non-parametric analysis of variance was used to compare both subjective and objective data.

\begin{figure}[htbp]
     \centering
     \begin{subfigure}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/hapticacc.png}
        \caption{ }
        \label{fig:hapticacc}
     \end{subfigure}
     \hspace{3em}
     \begin{subfigure}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/hapticeff.png}
        \caption{ }
        \label{fig:hapticeff}
     \end{subfigure}
     \hspace{3em}
     \begin{subfigure}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/hapticunder.png}
        \caption{ }
        \label{fig:hapticunder}
     \end{subfigure}
     \caption{Objective results of the haptic feedback characterization study.}
     \label{fig:haptic}
\end{figure}

% Understanding: vibro > none (Z = 2.10, p = 0.036), pneu > none (Z = 2.30, p = 0.021)
% Efftive: vibro > none (Z = 4.04, p < 0.001), pneu > none (Z = 2.64, p < 0.01)
% Deviation: vibro < none (Z = 5.40, p < 0.001), pneu < none (Z = 6.19, p < 0.001)

Statistical analysis results revealed a significant effect of the haptic feedback method on angle deviation, effective time, and understanding time, as shown in Fig~\ref{fig:haptic} $(p < 0.05)$. 
The increased angle deviation in \textbf{None}, compared to \textbf{Vibro} $(Z = 5.40, p < 0.001)$ and \textbf{Pneu} $(Z = 6.19, p < 0.001)$ verifies the supplemental haptic feedback' effect in enhancing the rehabilitation performance.
Both \textbf{Vibro} $(Z = 4.04, p < 0.001)$ and \textbf{Pneu} $(Z = 2.64, p < 0.01)$ outperformed \textbf{None} in helping users remain stable during the holding phase, indicated by their longer effective time.
Both \textbf{Vibro} $(Z = 2.10, p = 0.036)$ and \textbf{Pneu} $(Z = 2.30, p = 0.021)$ showed an increase in understanding time due to the extra time needed for actuation and for users to process the haptic motion guidance.
Fig~\ref{fig:haptic} shows no significant effect of other factors on the objective metrics. 
% The angle deviation for both vibrotactile and pneumatic feedback is smaller than no haptic feedback $(p < 0.05)$. 
% This verifies the supplemental haptic feedback' effect in enhancing the angular accuracy of motion guidance.
% The effective time, which is the time in which the user remained relatively stable, with vibrotactile feedback is longer than no haptic feedback $(p < 0.05)$.
% The understanding time for both vibrotactile and pneumatic feedback is longer than no haptic feedback $(p < 0.05)$. 
% This is due to the extra time needed to actuate the feedback and for users to understand the haptic motion guidance.


% $(p < 0.05)$
% Acc: None > Vibro, None > Pneu
% Eff: Vibro > None
% Under: None < Vibro, None < Vibro

% \textit{The haptic guidance did not increase understanding time and thus did not add extra cognitive load to users.}
% Statistical analysis results showed no significant difference between \textbf{None} $(M = 15.38 , SD = 13.00)$, \textbf{Vibro} $(M = 18.81, SD = 17.48)$ and \textbf{Pneu} $(M = 19.81, SD = 19.55)$.
% % Understanding time:
% % No significance found

% \textit{Haptic guidance could help users perceive their motion more accurately.}
% The test results showed significant difference on angle accuracy $({\chi}^2 = 41.55, p < 0.05)$. 
% Post-hoc tests showed significant difference between
% \textbf{None} $(M = 5.74, SD = 4.93)$ and \textbf{Vibro} $(M = 2.08, SD = 1.46)$ $(p < 0.05)$, 
% \textbf{None} $(M = 5.74, SD = 4.93)$ and \textbf{Pneu} $(M = 2.44, SD = 2.08)$ $(p < 0.05)$.
% Angle accuracy:
% significant difference (${\chi}^2=36.82, p<0.001$), post-hoc shows that it's between A(M = 5.74, SD = 4.93) and B(M = 2.08, SD = 1.46) ($p<0.001$), A(M = 5.74, SD = 4.93) and C(M = 2.44, SD = 2.08) ($p<0.001$)

% \textit{Users could maintain their motion more stable with haptic guidance.}
% The test results showed significant difference on angle accuracy ${\chi}^2 = 17.35, p < 0.05)$. 
% Post-hoc tests showed significant difference between
% \textbf{None} $(M = 5.76, SD = 4.02)$ and \textbf{Virbo} $(M = 7.02, SD = 3.79)$ $(p < 0.05)$, 
% \textbf{None} $(M = 5.76, SD = 4.02)$ and \textbf{Pneu} $(M = 6.59, SD = 3.99)$ $(p < 0.05)$.
% % Time proportion
% significant difference (${\chi}^2=17.35304, p<0.001$), post-hoc shows that it's between A($M=5.761, SD=4.020$) and B($M=7.019, SD=3.787$) ($p<0.001$), B($M=7.019, SD=3.787$) and C($M=6.586, SD=3.992$) ($p<0.05$)

\begin{figure}[htbp]
     \centering
     \begin{subfigure}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/hapticinf.png}
        \caption{ }
        \label{fig:hapticinf}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/hapticperp.png}
        \caption{ }
        \label{fig:hapticperp}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/hapticmot.png}
        \caption{ }
        \label{fig:hapticmot}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/hapticstr.png}
        \caption{ }
        \label{fig:hapticstr}
     \end{subfigure}
     \begin{subfigure}{0.19\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/hapticove.png}
        \caption{ }
        \label{fig:hapticove}
     \end{subfigure}
     \caption{Subjective results of the haptic feedback characterization study.}
     \label{fig:hapticsub}
\end{figure}


% Information Presentation: None < Vibro (Z = 2.23, p = 0.025), Pneu < Vibro (Z = 2.27, p = 0.023)
% Self Perception: None > Pneu (Z = 2.03, p = 0.042), Vibro > Pneu (Z = 2.12, p = 0.034)
% Motivated: None < Vibro (Z = 2.12, p = 0.034)
% Stress: None < Vibro (Z = 2.00, p = 0.046)
% Overall: None < Vibro(Z = 2.07, p = 0.038), None < Pneu (Z = 2.00, p = 0.044)

The subjective results showed a significant effect of the haptic feedback method on all subjective metrics, as shown in Fig~\ref{fig:hapticsub}.
\textbf{Vibro} was rated higher on information presentation compared to \textbf{None} $(Z = 2.23, p = 0.025)$ and \textbf{Pneu} $(Z = 2.27, p = 0.023)$.
Both \textbf{Vibro} $(Z = 2.12, p = 0.034)$ and \textbf{None} $(Z = 2.03, p = 0.042)$ were better on self perception compared to \textbf{Pneu}.
Participants explained in the interview that the intense vibrations convey clear haptic instructions, whereas the pneumatic feedback is slower and more subtle.
This created some confusion for the participants when using pneumatic feedback to convey rapidly changing motions, especially when the participants were fluctuating a lot during the holding phase.

Results revealed that compared to \textbf{None}, participants were more motivated $(Z = 2.12, p = 0.034)$ and also more stressed $(Z = 2.00, p = 0.046)$ with \textbf{Vibro}. 
% They also experienced a higher level of stress when exercising with vibrotactile feedback $(p < 0.05)$.
This was due to intense vibrations throughout the reaching phase and participants' knowledge that fluctuations during the holding phase would trigger vibration "warnings," which brought a numbing sensation.
They thus felt stressed to speed up their exercise and to reduce fluctuations.
Overall, participants preferred \textbf{Vibro} $(Z = 2.07, p = 0.038)$ and \textbf{Pneu} $(Z = 2.00, p = 0.044)$ over \textbf{None} while exercising.
This indicates that despite a mildly increased understanding time, participants found haptic feedback helpful in general in providing motion guidance and awareness.

In the interview, half of the participants preferred vibrotactile due to its intense and instantaneous response, while pneumatic airbags took longer to inflate.
The rest liked pneumatic feedback's soothing, supportive, and pseudo-kinesthetic sensation.




% \textit{Users could receive the guidance information better with haptic guidance, especially with vibrotactile guidance.}
% The statistical results showed significant difference on information presentation $({\chi}^2 = 6.62, p < 0.05)$.
% Post-hoc tests showed significant difference between 
% \textbf{None} $(M = 3.64, SD = 1.12)$ and \textbf{Vibro} $(M = 4.55, SD = 0.69)$ $(p<0.05)$, 
% \textbf{None} $(M = 3.64, SD = 1.12)$ and \textbf{Pneu} $(M = 4.18, SD = 1.17)$ $(p<0.05)$,
% and \textbf{Vibro} $(M = 4.55, SD = 0.69)$ and \textbf{Pneu} $(M = 4.18, SD = 1.17)$ $(p<0.05)$.
% Q2: significant difference (${\chi}^2=8.72000, p<0.05$), post-hoc shows that it's between A($M=3.636, SD=1.120$) and B($M=4.545, SD=0.688$) ($p<0.05$), B($M=4.545, SD=0.688$) and C($M=3.818, SD=0.982$) ($p<0.05$)
% Q3: significant difference (${\chi}^2=8.40000, p<0.05$), post-hoc shows that it's between A($M=4.182, SD=0.751$) and B($M=4.909, SD=0.302$) ($p<0.01$), B($M=4.909, SD=0.302$) and C($M=4.364, SD=0.674$) ($p<0.05$)
% Q4: significant difference (${\chi}^2=8.85714, p<0.05$), post-hoc shows that it's between A($M=4.545, SD=1.214$) and C($M=4.182, SD=1.168$) ($p<0.05$), B($M=4.818, SD=0.405$) and C($M=4.182, SD=1.168$) ($p<0.01$)

% Q6: significant difference (${\chi}^2=6.61538, p<0.05$), post-hoc shows that it's between A($M=4.455, SD=0.820$) and B($M=5.000, SD=0.000$) ($p<0.01$)

%The assessment of the questions related to the user's self-perception indicates significant difference between conditions in the question "To what extent did you know how your current posture" (p < 0.05), and it prefers "visual + vibrotactile feedback" over the baseline, according to post-hoc tests(p<0.05). 

% \textit{Users were more motivated with the vibrotactile guidance.}
% The statistical results showed significant difference on motivation gradings $({\chi}^2 = 6.35, p < 0.05)$.
% Post-hoc tests showed significant difference between 
% \textbf{None} $(M = 4.00, SD = 1.10)$ and \textbf{Vibro} $(M = 4.73, SD = 0.47)$ $(p<0.05)$.

% Q10: significant difference (${\chi}^2=6.34783, p<0.05$), post-hoc shows that it's between A($M=4.000, SD=1.095$) and B($M=4.727, SD=0.467$) ($p<0.05$)

%The assessment of the questions related to motivation indicates significant difference between conditions in the question "To what extent were you motivated to finish the task" (p < 0.05), and it also prefers "visual + vibrotactile feedback" over the baseline, according to post-hoc tests (p<0.05).

% \textit{Users liket the vibrotactile guidance better than the pneumatic one.}
% Statistical results shoed significant difference between 
% \textbf{Vibro} $(M = 4.22, SD = 0.84)$ and \textbf{Pneu} $(M = 3.42, SD = 0.45)$ $(p < 0.05)$.
% % Q14: significant difference ($W=0.0, p<0.01$) between B($M=4.200, SD=0.837$) and C($M=3.200, SD=0.447$)
% % Q16: significant difference ($W=0.0, p<0.05$) between B($M=4.600, SD=0.548$) and C($M=4.000, SD=1.000$)

% \textit{Users generally liked the haptic guidance in this experiment.}
% The statistical results showed significant difference on overall assessments $({\chi}^2 = 8.38, p < 0.05)$.
% Post-hoc tests showed significant difference between 
% \textbf{None} $(M = 4.00, SD = 0.27)$ and \textbf{Vibro} $(M = 4.82, SD = 0.41)$ $(p<0.05)$, 
% \textbf{None} $(M = 4.00, SD = 0.27)$ and \textbf{Pneu} $(M = 4.55, SD = 0.69)$ $(p<0.05)$.
% % Q13: significant difference (${\chi}^2=8.37500, p<0.05$), post-hoc shows that it's between A($M=4.000, SD=1.265$) and B($M=4.818, SD=0.405$) ($p<0.01$), A($M=4.000, SD=1.265$) and C($M=4.545, SD=0.688$) ($p<0.05$)

%Finally, the overall ratings indicates significant difference between conditions (p<0.05), preferring the two conditions with haptic feedback over the baseline, according to post-hoc tests (p<0.05). The assessment of the questions related to stress did not present significant differences.

% We also compared the two forms of haptic feedback based on questions related to the effectiveness of haptic feedback and the post-experiment interview. The Wilcoxon signed-rank test was applied to the questions.


%and significant difference was found in the question "To what extent did you think the feedback was acute and pinpoint" and "To what extent did you think the feedback aided you", both in favor of vibrotactile feedback (p<0.05). 
% During the interview, subjects pointed out that when consistent feedback was needed, the mild feedback provided by pneumatic airbags was more comfortable compared to vibration.
% Users also commented that the vibrotactile actuators could provide real-time feedback, while pneumatic feedback was delayed by the process of inflation and deflation.


% valuable characteristics of different feedback during the interview. 
% 1. when consistent feedback is needed, the mild feedback provided by pneumatic airbags is more comfortable compared to vibration. 
% 2. the vibrotactile actuators can provide real-time feedback, while pneumatic feedback is delayed by the process of inflation and deflation.


% Similar with the last experiment, the objective data consists of the angle between the thigh and the floor surface and the angle between the thigh and the lower leg, used to evaluate the participants’ correctness of the motion. 
% In this experiment, we also recorded the time taken to complete the motion and the time within an acceptable range of correctness while the subject is holding steady in order to evaluate how haptic feedback facilitates the rehabilitation process. 
% The Friedman test along with the Conover post-hoc test was applied. 
% Our results concerning the correctness of the motion reveal significant differences (p<0.005) in all motions (straight leg raises, prone leg raises, and bed-supported knee bends), preferring the two conditions with haptic feedback over the baseline, according to post-hoc tests (p<0.05). 
% In terms of completion time, significant differences (p<0.005) is found in straight leg raises and bed-supported knee bends, and post-hoc test indicates that both the baseline and "visual + vibrotactile feedback" took significantly shorter time to finish than "visual + pneumatic feedback" (p<0.05). 
% This supports the result of the interview, which mentioned the delay of pneumatic feedback. In terms of the time within a range of correctness, significant differences (p<0.005) is found in straight leg raises and prone leg raises. 
% According to post-hoc tests, pneumatic feedback allows subjects to hold still for a longer time than the baseline condition (p<0.005) during straight leg raises, and both kinds of haptic feedback allows subjects to hold still for a longer time than the baseline condition (p<0.05) during prone leg raises. 
% This suggests that under haptic feedback conditions, people were able to enhance their stability while sticking to the correct motion.

% According to our results, both objective and subjective data show haptic feedback's advantage over pure visual system: it enhances the correctness of the poses, the users' ability to hold the correct pose, and has a better overall rating. 
% Within the two kinds of haptic feedback, vibrotactile feedback seems to have more advantage, giving the users better self-perception and motivation compared to the baseline, and offering real-time feedback. 
% However, we should not neglect the fact that some users reported that pneumatic feedback is more comfortable when exerting consistent feedback, especially when the system is applied to medical purposes. 
% In conclusion, Vibroactile gives a more sudden and intense sensation and can be disturbing if actuated for a long time. 
% On the other hand, pneumatic is slow in actuation yet provides a soothing, pseudo-kinesthetic sensation.

% Thus, we decided to synthesize both vibrotactile and pneumatic feedback into the system. 
% Starting from the ready position, pneumatic feedback is used when the user is reaching for the target position, as it may take a long period of time for patients; vibrotactile feedback is used for the holding-still process, where more acute and real-time feedback is needed for the user to adjust his or her moves.




%The assessment of the questions concerning information presentation, "To what extent did you how to exert your force", "To what extent did the information conveyed by the system help you", and "To what extent did you understand the information conveyed by the system" reveals significant difference between conditions (p<0.05). 
%Post-hoc tests show that "visual + vibrotactile feedback" is preferred over the other two conditions (p<0.05) in the first two questions, while both the baseline and "visual + vibrotactile feedback" is preferred over "visual + pneumatic feedback" in the last question (p<0.05). 
\subsection{Finalizing the haptic feedback}
Based on the study results, we finalized the haptic feedback in \systemname and implemented the haptic feedback functionalities. 

\subsubsection{Vibrotactile and pneumatic haptic feedback mechanism}
We combine vibrotactile and pneumatic feedback's respective advantages in our implementation of \systemname. 
Specifically, we mapped these two haptic feedback methods to different phases of a movement. 
Pneumatic feedback is provided in the reaching phase. 
The gradually exerted pressure on the skin notifies the user to slowly, and thus safely, reach the target pose. 
Once \systemname detects that the user has stabilized and starts the holding phase, vibrotactile feedback is provided to supervise the user's adherence target pose during the holding phase.
The corresponding vibrator is actuated when the user goes below or above the acceptable holding range.
Upon receiving instantaneous and intense "warnings," the user can timely adjust his/her pose.
When the 10 seconds countdown stops, haptic feedback is paused until the next movement starts. 

\subsubsection{Fabrication}
We combined the vibrator and the air compartment into one haptic feedback module with two such modules on each strap.
We designed and 3D-printed cases to assemble each pair of vibrators and air compartments and to mount the assembly onto the strap (Fig~\ref{fig:hapticcombine}).

The vibrators and the relay, which control the pneumatic system, are altogether controlled by an Arduino Mega.
The Arduino Mega is connected to a computer and reads commands through a serial port.
We 3D printed a box (278mm in length, 246mm in width, and 98mm in height) to assemble the relay, Arduino Mega, regulated power supply, step-down converter, and 8 micro-pumps together compactly so that \systemname can be easily mobilized.
Fig~\ref{fig:implementation} demonstrates the assembled box. 

\begin{figure}[htbp]
     \centering
     \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/haptic.jpg}
        \caption{ }
        \label{fig:hapticcombine}
     \end{subfigure}
     \hfill
     \begin{subfigure}{0.66\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/characterization/implementation.png}
        \caption{ }
        \label{fig:implementation}
     \end{subfigure}
     \caption{(a): We assemble each pair of vibrators and air compartments on a strap. (b): The entire haptic system in a 3D printed box.}
\end{figure}


==> sections/background.tex <==
\section{background}
% the importance of rehab to TKA patients
Total knee anthroplasty (TKA) remains the most effective treatment for end-stage arthropathy of the hip and knee joints [Wang]. Rehabilitation is a crucial part of recovery after TKA which typically begins in the hospital and resumes at home after discharge. For such lower-limb impairments studies have shown that if performed in a quality manner, repetitive and sufficient motor learning centered rehabilitation could improve post-surgery motor abilities as well as health-related quality of life[64, 120, 121, 132 from Jung]. To ensure that the rehabilitation is carried out in a therapeutically appropriate way licensed therapists are needed to instruct, supervise, and control such sessions in a clinical setting and continue to monitor at-home remote rehabilitation after discharge.

% the need for remote TKA rehab in China 
The number of TKA patients is rapidly growing in China with a annual case number of 53,880 in 2011 to 374,833 in 2019 [Feng]. Yet only a limited number of hospitals in China provide post-surgery rehabilitation services and there is a dire shortage of qualified therapists domestically. The lack of appropriate therapeutic rehabilitation was exacerbated by the COVID-19 pandemic which discouraged people from going or staying in the hospital. This kept large number of post TKA patients from receiving proper motor ability recovery rehabilitation and thus from a successful post-surgery recovery to a quality life. In light of this, the need for remote and self-monitored rehabilitation is in the rise in the hope that such method could provide professional therapeutic guidance in safe and comfortable home environment. At the same time if the remote system can replace part of clinical rehabilitation the hospitals can maximize their medical resources utility by discharging the TKA patients quicker.
